Robust Time Series Dissimilarity Measure for Outlier Detection and Periodicity Detection

Dynamic time warping (DTW) is an effective dissimilarity measure in many time series applications. Despite its popularity, it is prone to noises and outliers, which leads to singularity problem and bias in the measurement. The time complexity of DTW is quadratic to the length of time series, making it inapplicable in real-time applications. In this paper, we propose a novel time series dissimilarity measure named RobustDTW to reduce the effects of noises and outliers. Specifically, the RobustDTW estimates the trend and optimizes the time warp in an alternating manner by utilizing our designed temporal graph trend filtering. To improve efficiency, we propose a multi-level framework that estimates the trend and the warp function at a lower resolution, and then repeatedly refines them at a higher resolution. Based on the proposed RobustDTW, we further extend it to periodicity detection and outlier time series detection. Experiments on real-world datasets demonstrate the superior performance of RobustDTW compared to DTW variants in both outlier time series detection and periodicity detection.

==> backup_3-methodology.tex <==
\section{Methodology}\label{section:method}

%In this section, we describe the detailed framework of our proposed RobustDTW algorithm and its multi-level extension for efficient computation.
%  and missing data manipulation


% Model Overview
% \subsection{Model Overview} \label{subsection:robustdtw} 
% https://yuque.antfin-inc.com/d3algo/alg-study/rdtw
\subsection{Proposed RobustDTW Algorithm} \label{subsection:robustdtw} 

To make DTW robust to noise and outliers while preserving its flexibility of dynamic index matching, we employ the robust trend to filter out the noises and outliers. Specifically, we propose to estimate the time warp function and detrend TS in an alternating manner. We iteratively conduct the following operations: (1) fix the time warp function and estimate the detrended TS $u$ and $v$; (2) fix the estimated detrended TS $u$ and $v$, and estimate the time warp function $\varphi(t)$ based on $u$ and $v$. 

To speedup the computation of proposed RobustDTW, we utilize the similarity of the shapes and alignments of TS pairs among different resolutions, and combine alternating of DTW align adjustment and trend estimate with the progress from low resolution to high resolution. %To this end, we merge inner loop (progress resolution) with outer loop (alternating DTW alignment and trend estimate) to speedup the calculations. 
During this multi-level progress, low resolution trend results are the starting values for high resolution estimation, as low resolution index alignment can suggest the constraint of path searching space for high resolutions. 
% We summarize this detailed procedure of the proposed alternating algorithm in Alg. \ref{alg:alternative}, followed by detailed description of each step.
We summarize the detailed procedure of the proposed alternating algorithm in Alg.~\ref{alg:multi-level}, followed by detailed description of each step. In our empirical studies, we found that three iterations are often enough for convergence.



\iffalse
% algorithm of alternating multi-level framework
\floatname{algorithm}{Algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}

\begin{algorithm}
\caption{RobustDTW Algorithm}
\label{alg:alternative}
\begin{algorithmic}
\REQUIRE $\textbf{x}$, $\textbf{y}$, input TS; $\lambda^{j}_i$ regularization parameters.
\ENSURE Normalized robust DTW distance

\STATE \textbf{Step 1:} \text{Robust Self-Detrending}
\INDSTATE[1] normalize x, y
\INDSTATE[1] $\mathbf{a} = \text{argmin}_\mathbf{u} \ g_{\gamma}(\mathbf{x}, \mathbf{u}) + \lambda^{\textrm{\textrm{self}}}_1||\mathbf{D}^{(1)}\mathbf{u}||_1 $
\INDSTATE[1] \hspace{18pt}$ + \lambda^{\textrm{\textrm{self}}}_2||\mathbf{D}^{(2)}\mathbf{u}||_1$
\INDSTATE[1] $\mathbf{b} = \text{argmin}_\mathbf{v} \ g_{\gamma}(\mathbf{y}, \mathbf{v}) + \lambda^{\textrm{\textrm{self}}}_1||\mathbf{D}^{(1)}\mathbf{v}||_1 $
\INDSTATE[1] \hspace{18pt}$ + \lambda^{\textrm{\textrm{self}}}_2||\mathbf{D}^{(2)}\mathbf{v}||_1$
\STATE \textbf{Step 2:} \text{Time Warping Alignment}
\INDSTATE[1] In the first iteration, use \textbf{a}, \textbf{b} as input for DTW to generate warping path. In subsequent iterations, use updated \textbf{u}, \textbf{v} to generate warping path.
\STATE \textbf{Step 3:} \text{Temporal Graph Detrending}
\INDSTATE[1] Get warping path from step 2 and update \textbf{u}, \textbf{v} with graph detrending:
\INDSTATE[1] $\mathbf{u, v} = \text{argmin}_{\mathbf{u},\mathbf{v}} \ \frac{1}{2} \|[\mathbf{u}; \mathbf{v}]- [\mathbf{a}; \mathbf{b}]\|_2^2$ 
\INDSTATE[1] \hspace{28pt}$ + \lambda^{\textrm{\textrm{GD}}}_1 \| D^{(1)}_\textrm{G} [\mathbf{u}; \mathbf{v}]\|_1 + \lambda^{\textrm{\textrm{GD}}}_2 \| D^{(2)}_\textrm{G} [\mathbf{u}; \mathbf{v}]\|_1$

\STATE \textbf{Step 4:} \text{Repeat steps 2-3, until converge}
\INDSTATE[1] Repeat Steps 2-3 with updated warping path and trend estimates \textbf{u} and \textbf{v}
\STATE \textbf{Step 5:} \text{Return results}
\INDSTATE[1] use estimated trend \textbf{u}; \textbf{v} and their warping path to get cumulative distance then divide by the length of the TS.

% https://tex.stackexchange.com/questions/360418/alignment-of-multlined-equations-in-algorithm

\end{algorithmic}
\end{algorithm}
\fi

% \vspace{-5cm}
{\hspace{-5mm}\bf Step 1: Robust Self-Detrending}\\
To roughly remove the effects of outliers and noise, we first adopt robust trend filtering for individual TS. 
Let denote the TS of length $n$ as $\mathbf{y}=[y_1, y_2, \cdots, y_{n}]^T$, which can be decomposed into trend and residual components ~\cite{alexandrov2012review}
\vspace{-2mm}
\begin{equation}\label{eq:Univariate} 
y_t = \tau_t + r_t \quad\text{or}\quad \mathbf{y} = \boldsymbol{\tau} + \mathbf{r}
\vspace{-2mm}
\end{equation}
where $\boldsymbol{\tau}=[\tau_1, \tau_2, \cdots, \tau_{n}]^T$ denotes the trend component, and $\mathbf{r} = [r_1, r_2, \cdots, r_{n}]^T$ denotes the residual component, which contains noises and outliers. 
%Since we consider the TS faced in real-world applications, 
% the trend component may contains both slow trend change and abrupt trend change, while the residual component may contains both noise and outliers.
% Note that in this subsection we only consider a an univariate TS. In the following discussion if multiple TS are considered, we use a superscript like $\mathbf{y}^{(i)}$ to denote the $i$th TS. 
We adopt the RobustTrend filter~\cite{wen2019robusttrend} to detrend TS, i.e., estimate $\boldsymbol{\tau}$, as it captures both slow and abrupt trend changes while robust to outliers. 


% algorithm of alternating multi-level framework
\floatname{algorithm}{Algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}

\begin{algorithm}[t]
\caption{RobustDTW with Multi-Level Framework}
\label{alg:multi-level}
\begin{algorithmic}
\REQUIRE $\textbf{x}$,  $\textbf{y}$, input TS; $\lambda^{j}_i$ regularization parameter configurations; $t$, iteration times; $r$, radius.
\ENSURE normalized RobustDTW distance.

\STATE \textbf{Step 1:} \text{\bf Robust self-detrending}: apply RobustTrend on \textbf{x} and \textbf{y}, respectively, to get \textbf{a} and \textbf{b} as the detrend output.

\STATE \textbf{Step 2:} \text{\bf Multi-Level Representation}: recursively down sample \textbf{a} and \textbf{b}, and record the intermediate results.

\STATE \textbf{Step 3:} \text{\bf Projection and Upsampling}: in the first iteration, run FastDTW~\cite{salvador2007toward} to get warping path and use the highest level down-sampled \textbf{a} and \textbf{b} as initial trend estimates; otherwise, perform upsample trend estimates and project DTW warping path with from previous level to current level.
\STATE \textbf{Step 4:} \text{\bf Time  Warping  Alignment}: refine warping alignment by DTW with projected constraint from step 3.

\STATE \textbf{Step 5:} \text{\bf Temporal Graph Detrending}: generate graph from updated warping from step 4 and refine graph detrending with updated trend estimates.
\STATE \textbf{Step 6:} \text{Repeat Steps (3)-(5) until lowest level.}
\STATE \textbf{Step 7:} \text{Return normalized RobustDTW distance.}
% https://tex.stackexchange.com/questions/360418/alignment-of-multlined-equations-in-algorithm
% \INDSTATE[1] for loop

\end{algorithmic}
\end{algorithm}


\iffalse
It extracts trend by minimizing the following objective function
\begin{equation}\label{eq:robust_trend} 
g_{\gamma} (\mathbf{y} - \boldsymbol{\tau}) 
+ \lambda_1 || \mathbf{D}^{(1)}\boldsymbol{\tau} ||_1
+ \lambda_2 || \mathbf{D}^{(2)}\boldsymbol{\tau} ||_1,
\end{equation}
where $g_{\gamma} (\mathbf{x})=\sum_i g_{\gamma} (x_i)$ is the summation of elementwise Huber loss function with each element as
\begin{equation}\label{eq:huber_loss} 
 g_{\gamma} (x_i) =
\begin{cases} 
\frac{1}{2} x_i^2,       & |x_i| \leq \gamma\\
\gamma|x_i|- \frac{1}{2} \gamma^2, & |x_i| > \gamma
\end{cases}.
\end{equation}
And the ${D}^{(1)}\in \mathbb{R}^{(N-1)\times N}$ and ${D}^{(2)}\in \mathbb{R}^{(N-2)\times N}$ are the first-order and second-order difference matrix, respectively: 
\begin{equation} \label{eq:Dk}\notag
\resizebox{1.0\hsize}{!}{$
\mathbf{D}^{(1)} =  
\begin{bmatrix}
1 & -1\\
  & 1& -1\\
& &\ddots\\
&&1&-1
\end{bmatrix},
~\mathbf{D}^{(2)} = 
\begin{bmatrix}
1 & -2 &1&\\
&1&-2&1&\\
&&&\ddots\\
&&&1&-2&1
\end{bmatrix}.
$}
\end{equation}
In RobustTrend filter, the Huber loss brings better robustness to outliers compared to commonly used sum-of-squares loss, while the 1st and 2nd order difference operators in the regularization terms can capture both abrupt and slow trend changes. Therefore, the two input TS \textbf{x} and \textbf{y} after detrending operations can be written as
\begin{equation}\label{eq:pre_detrend}\notag
\begin{split}
\mathbf{u} & = \text{argmin}_u \ g_{\gamma} (\mathbf{x}, \mathbf{u}) + \lambda_1^{\textrm{self}}||\mathbf{D}^{(1)}\mathbf{u}||_1 + \lambda_2^{\textrm{self}}||\mathbf{D}^{(2)}\mathbf{u}||_1, \\
\mathbf{v} & = \text{argmin}_v \ g_{\gamma} (\mathbf{y}, \mathbf{v}) + \lambda_1^{\textrm{self}}||\mathbf{D}^{(1)}\mathbf{v}||_1 + \lambda_2^{\textrm{self}}||\mathbf{D}^{(2)}\mathbf{v}||_1.
\end{split}
\end{equation}

\fi
% where $L$ is the empirical loss function. We can choose sum-of-squares loss function for simplicity, i.e., $L(\mathbf{x}, \mathbf{u})=\|\mathbf{x}-\mathbf{u}\|_2^2$ ; we can also use the Huber loss for better robustness; $\mathbf{D}^{(1)}$ and $\mathbf{D}^{(2)}$ are the 1st and 2nd order difference operators, and their detailed definitions can be found below in subsection~\ref{subsection:diff}.

{\hspace{-5mm}\bf Step 2: Multi-Level Representation}\\
Multi-level representations can be achieved by down sample detrended TS from Step 1. E.g., the level 1 representation is the original detrended TS, and down sample level 1 by factor of 2 to generate the level 2 representation. This procedure is conducted until the level $t$ representation is obtained, where $t$ is the total levels in the framework. Note that higher level representations correspond to lower resolution TS.

{\hspace{-5mm}\bf Step 3: Projection and Upsampling}\\
In first iteration, starting from level $t$ TS, call FastDTW~\cite{salvador2007toward} to get warping index alignment and use current level representations as the base trend estimation; In the subsequent iterations, up-sample previous level's warping path by 2 and add extra searching width defined by parameter radius to generate the searching constraint, which is called projection. Also, we perform upsampling previous level trend estimation to current level.

{\hspace{-5mm}\bf Step 4: Time Warping Alignment}\\
Refine the warping path by running DTW at current level with projected warping constrain to obtain the time warp function $\varphi(t)$, which corresponds to the mapping of index from \textbf{x} to \textbf{y}
% After self-detrending, we apply the standard DTW  algorithm %by recursively calling Eq.~\eqref{eq:DTW} on $\mathbf{u}$ and $\mathbf{v}$ 
% to obtain the time warp function $\varphi(t)$, which corresponds to the mapping of index from TS \textbf{x} to \textbf{y}.
%\begin{equation}\label{eq:DTW}
%\begin{aligned}
%\text{D}(i, j) = \text{Dist}(i, j) + \text{min} {}[{} & %\text{D}(i-1,j), \text{D}(i, j-1), \\
%                                                      & %\text{D}(i-1, j-1)],
%\end{aligned}
%\end{equation}
%where \text{D}($i$, $j$) is the cumulative distance and the \text{Dist}($i$, $j$) is the local distance between point $i$ and $j$.
% Note that, this step can be extended in a  multi-level way for efficient computation and missing data manipulation, which will be described in detail later.

% in tsubsection ~\ref{subsection:multi}.
% In the future we can estimate the time warp function $\varphi(t)$ by solving an optimization problem, as Stephen Boyd did in his 2019 paper [Boyd2019DTW](https://arxiv.org/pdf/1905.12893.pdf).



% \subsubsection{Difference Operator and Graph Detrending} \label{subsection:diff}
% Here we introduce the concept of Difference Operator in general temporal-spatial and graph detrending.

% The detrending can be considered as a type of nonparametric regression. In the literature, the detrending has been successfully applied in trend filtering and graph trend filtering. Some advantages of trend filtering are summarized as local adaptiveness, computational efficiency and analysis regularization. 

% \subsubsection{1. Univariate Temperal Difference Operator}

{\hspace{-5mm}\bf Step 5: Temporal Graph Detrending}\\
% \subsubsection{3. Graph Detrending for Multiple Related TS}\label{sssec:detrending}
In this step, we aim to estimate the detrended TS $\mathbf{u}$ and $\mathbf{v}$ more accurately by considering not only its neighbors within itself but also its similar peer TS. 
%In the following, we will show how to extend the idea of graph detrending~\cite{wang2016trend} to multivariate TS.
%pair of TS to achieve this.


Let $G = (V, E)$ be an graph, with vertices $V = \{1, \cdots, n\}$ and undirected edges $E = \{e_1, \cdots, e_s\}$, and suppose that we observe $\mathbf{y} = [y_1,\cdots, y_n]^T \in R^n$ over each node. Similarly, the $k$th order graph trend filtering estimates $\boldsymbol{\tau}=[\tau_1, \cdots, \tau_n]^T$ can be obtained by solving: 
\vspace{-2mm}
\begin{equation}\label{eq:GTF} 
\text{argmin}_{\tau\in R^n} \ \frac{1}{2} \|\mathbf{y}-\boldsymbol{\tau}\|_2^2 + \lambda \| \Delta^{(k+1)} \boldsymbol{\tau} \|_1,
\vspace{-2mm}
\end{equation}
where $\Delta^{(k+1)}$ is the graph difference operator of order $k+1$. 
When $k=0$, the 1st order graph difference operator $\Delta^{(1)}$ penalizes all local differences on all edges as
% \begin{equation}\label{eq:gdo}
$\|\Delta^{(1)} \boldsymbol{\tau} \|_1 = \sum_{(i,j)\in E} | \tau_i - \tau_j |$. 
% \end{equation}
Note that we can represent $\Delta^{(1)}$ in a matrix form as $\Delta^{(1)}\in \{-1,0,1\}^{s\times n}$ where $s=|E|$, i.e., number of edges. Specifically, let $e_{\ell}=(i,j)$, then $\Delta^{(1)}$ has the $\ell$th row as
% \begin{equation}\label{eq:gdo-row}
$\Delta^{(1)}_{\ell} = [0, \cdots, -1, \cdots, 1, \cdots, 0]$,
% \end{equation}
i.e., $\Delta^{(1)}_{\ell}$ has -1 at the $i$th position, and 1 at the $j$th position. Similar to trend filtering on univariate TS, we can define the higher order graph difference operators recursively. In particular, the graph difference operators defined above reduce to the ones defined on the univariate TS in which $V=\{1,2,\cdots,n\}$ and $E=\{(i,i+1): i=1,2,\cdots,n-1\}$. 

% Take the classical H-P trend filtering on univariate TS data as an example, it can be considered as a specical case of graph trend filtering. Specifically, we build a graph where each node corresponds to a sample at a time point, and we create edge connecting nodes which corresponding to consecutive samples in the TS. Basically, we can build a chain graph on which the graph detrend filtering reduces to the standard univariate trend filtering. 

In this paper, we design a general temporal graph detrending for multivariate TS by extending the idea of the graph-based detrending in Eq.~\eqref{eq:GTF}. 
The key idea is to incorporate the relationship between TS in detrending which can also deal with the lagging effect adaptively. Another distinguishing feature is that we introduce weight for each edge in the graph, instead of only allowing binary weight as in \cite{wang2016trend}. 

% Therefore, we construct a graph $G_t$, where each node corresponds to a metric (or TS). Suppose there are $M$ TS denoted as $ts_1, ts_2, \cdots, ts_M$. We use $s_{ij}$ to denote the similarity between the $i$th TS and the $j$th TS. 
% % Note that we assume $s_{ij}$ could be negative to reflect that 
% In the multi-metric case, we denote the observed data in the matrix form $\mathbf{Y}=[\mathbf{y}_1, \mathbf{y}_2, \cdots, \mathbf{y}_M]^T\in R^{M\times N}$
% where $\mathbf{y}_i = [y_{i1}, y_{i2}, \cdots, y_{iN}]^T \in R^N$ denotes the $i$th TS.
% % . One challenge in multiple TS processing is the lagging effect, which means that the change of one TS can lead to the change of some other TS.
% % Main Point: in the detrending of multiple TS, we need to consider the pairwise similarity between different pairs of metrics (TS). In other words, instead of detrending each metrics independently, we consider the relationship between different metrics and perform detrending of them together. 
% Unlike the univariate case, in multiple TS detrending we construct a graph $G_t$, where each node corresponds to a metric (or TS). Suppose there are $M$ TS denoted as $ts_1, ts_2, \cdots, ts_M$. We use $s_{ij}$ to denote the similarity between the $i$th TS and the $j$th TS. 
% Note that we assume $s_{ij}$ could be negative to reflect that 
% In the multi-metric case, we denote the observed data in the matrix form $\mathbf{Y}=[\mathbf{y}_1, \mathbf{y}_2, \cdots, \mathbf{y}_M]^T\in R^{M\times N}$
% where $\mathbf{y}_i = [y_{i1}, y_{i2}, \cdots, y_{iN}]^T \in R^N$ denotes the $i$th TS.
% % , where 
% % \begin{equation}\label{eq:MultiTS1}
% % \mathbf{Y} = \begin{bmatrix} \mathbf{y}_1^T \\ \mathbf{y}_2^T \\ \vdots \\ \mathbf{y}_M^T
% % \end{bmatrix},
% % \end{equation}
% % \begin{equation}\label{eq:MultiTS2}
% % \mathbf{y}_i = \begin{bmatrix} y_{i1} \\ y_{i2} \\ \vdots \\ y_{iN}
% % \end{bmatrix}.
% % \end{equation}
% The trend components of $M$ metrics can also be represented as a matrix 
% $\mathcal{T}=[\mathbf{\tau}_1, \mathbf{\tau}_2, \cdots, \mathbf{\tau}_M]^T\in R^{M\times N}$
% where $\mathbf{\tau}_i = [\tau_{i1}, \tau_{i2}, \cdots, \tau_{iN}]^T \in R^N$.
% % $\mathcal{T}\in R^{M\times N}$:
% % \begin{equation}\label{eq:MultiTS3}
% % \mathcal{T} = 
% % \begin{bmatrix} 
% % \mathbf{\tau}_1^T \\ \mathbf{\tau}_2^T \\ \vdots \\ \mathbf{\tau}_M^T
% % \end{bmatrix},
% % \mathbf{\tau}_i=
% % \begin{bmatrix}
% % \tau_{i1} \\ \tau_{i2} \\ \vdots \\ \tau_{iN}
% % \end{bmatrix}.
% % \end{equation}
% Similar to our previous discussion, we can build a graph with $M\times N$ nodes, and perform detrending based on the difference operator on the graph. 
Specifically, we construct the graph of two TS based on the alignment at step 4. In the constructed graph $G$, we have $m+n$ vertices, and each vertex corresponds to a time point in $\mathbf{x}\in R^m$ and $\mathbf{y}\in R^n$. For notation simplicity, we denote the set of vertices as $E=\{x_1, x_2, \cdots, x_m, y_1, y_2, \cdots, y_n\}$. Next, we describe how to construct edges and their corresponding weights. Firstly, each vertex $x_t$ is connected its left neighbor $x_{t-1}$ and right neighbor $x_{t+1}$. Secondly, $x_t$ should be connected to its peer in $\mathbf{y}$, i.e., $y_{\varphi(t)}$. Thirdly, to avoid errors introduced in DTW of step 4, we construct more edges to improve robustness. For the edge $x_t \leftrightarrow y_{\varphi(t)}$, we introduce additional $4$ edges, including $x_t \leftrightarrow  y_{\varphi(t)-1}$, $x_t \leftrightarrow  y_{\varphi(t)+1}$, $x_{t-1} \leftrightarrow  y_{\varphi(t)}$, $x_{t+1} \leftrightarrow  y_{\varphi(t)}$, as illustrated in the Fig.~\ref{fig:3-graph-detrending}. Note that in Fig.~\ref{fig:3-graph-detrending} we only consider the direct one neighbor of $x_t$ and $y_{\varphi(t)}$. In practice, we can increase the size of the neighborhood based on the noises and outliers of data accordingly.%In terms of the weight of the graph, 
%We set the weight between neighbor as 1 and weight between peer to 0.2 heuristically. The weight between peers can also decay when the pairs are away from DTW alignment.
% In the later experiment we can borrow the idea from bilateral filtering to future improve the robustness and adaptness of our algorithm.
% ~\ref{subsection:diff}
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.6\linewidth]{figs/3_graph_detrending.png}
    \vspace{-2mm}
    \caption{\small Illustration of the graph construction between two TS. Each data points are connected not only to their neighbors in the same TS but also to their peers to the other TS which are aligned by DTW. The time stamp on \textbf{x} are $t-1$, $t$, $t+1$, and $\varphi$(t) is the mapping of index from \textbf{x} to \textbf{y}. So that the aligned points are $t-1$, $t$, $t+1$ on \textbf{x} to $\varphi(t-1)$, $\varphi(t)$, $\varphi(t+1)$ on \textbf{y}.}
    \label{fig:3-graph-detrending}
    \vspace{-2mm}
\end{figure}


After constructing the graph $G$ for a pair of TS, the designed temporal graph detrending is computed as:
\vspace{-2mm}
\begin{equation}\label{eq:graph_detrend}
\begin{aligned}
\mathbf{u, v}\!\!=\!\text{arg}\!\min\limits_{\mathbf{u, v}}\!\frac{1}{2} \|\mathbf{w}\!-\! [\mathbf{x}; \mathbf{y}]\|_2^2 \!+\!\! \lambda_1^{\textrm{GD}} \| D^{(1)}_\textrm{G} \!\mathbf{w}\|_1\!\!+\!\! \lambda_2^{\textrm{GD}} \| D^{(2)}_\textrm{G} \!\mathbf{w}\|_1,%\nonumber
\end{aligned}
\vspace{-2mm}
\end{equation}
% \begin{equation}\label{eq:DTW}
% \begin{aligned}
% \text{D}(i, j) = \text{Dist}(i, j) + \text{min} {}[{} & \text{D}(i-1,j), \text{D}(i, j-1), \\
%                                                       & \text{D}(i-1, j-1)],
% \end{aligned}
% \end{equation}
where $\textbf{w}=[\textbf{u}; \textbf{v}]$ is the concatenate of input $\textbf{u}$ and $\textbf{v}$, 
${D}^{(1)}_\textrm{G}$ and ${D}^{(2)}_\textrm{G}$ are the 1st and 2nd graph difference operators %defined on the weighted graph $G$ 
used to capture abrupt and slow trend changes.%, respectively, motivated by RobustTrend as Eq.~\eqref{eq:robust_trend}.

% We propose to use a modified version of the ADMM or MM? to solve the resulting optimization problem.
% May need some description on MM using L0.

%  , we define the graph difference operator described in subsection 3.
% Denote , i.e., ,  and then we can perform the graph detrending by solving the following optimization problem: 
\iffalse

\subsubsection{Iterative Processing}
% ~\ref{sssec:warp}  ~\ref{sssec:GD}
To achieve better performance, we repeat Steps 2 and 3 to update the time warp function and the trend estimates until convergence. In our empirical studies, we found that three iterations are often enough for convergence. After convergence, the two estimated TS and their alignments achieve a desirable trade-off which not only keeps close to original TS but also has the final alignment with lower DTW distance.

\subsection{RobustDTW with Multi-Level Framework}\label{subsection:multi}
% Combine multi-level and alternating
\subsubsection{Acceleration}
In the previous RobustDTW scheme, it calculates DTW distances multiple times due to the iterative procedure, which is not computationally efficient for long TS due to the quadratic time and space complexity of DTW.
A simple improvement is just replace DTW with FastDTW within each iteration. But still, it has one full alignment calculation at highest resolution per iteration.

% In FastDTW ~\cite{salvador2007toward}, the author uses a multilevel approach to accelerate DTW calculation with linear time and space complexity with three steps: 1) Coarsening - down sample (and smoothing at the same time) and shorten TS into a lower resolution representations, usually recursively by a factor of two. 2) Projection - find DTW alignment in the lower resolution, and use this warping path to "up sample" to two times higher resolution with additional width (called radius, as a hyper parameter) so that to create a warping constraint area for higher resolution. 3) Refinement - run DTW algorithm within this constraint and get a finer warping path. Then repeats 2) \text{\~{}} 3) until the highest resolution. This is an approximation to standard DTW with assumption that the lower resolution TS are similar to its higher level TS which means that the TS are smooth with only have lower frequency components.

% ToDO: read the details of FastDTW, then rewrite this subsection. 

% This multi-level methods is similar to continuation methods, which starts with smoother and shorter TS (or smoother loss function in continuation methods) and less computationally expensive, then gradually fine tune the results at finer structure. In many cases with appropriate radius, this smoothing and down sample process preserves enough information about the shape of the TS with a global view, followed by solving progressively finer version of the problem.

% To accelerate the computational speed of the proposed RobustDTW algorithm, we utilize the similarity of the shapes and alignments of TS pairs among different resolutions, and combine alternating of DTW align adjustment and trend estimate with the progress from low resolution to high resolution. To this end, we merge inner loop (progress resolution) with outer loop (alternating DTW alignment and trend estimate) to speed up the calculations. During this progress, low resolution trend results can be set as starting values for high resolution estimation, since low resolution index alignment can suggest the constraint of path searching space for high resolutions. 

% Add content in https://yuque.antfin-inc.com/d3algo/alg-study/xco6n2
This multi-level RobustDTW algorithm is summarized in Alg. \ref{alg:multi-level} and described below in detail:
(1) Robust Self-Detrending: Detrend TS at original highest resolution.
(2) \textbf{Multi-Level Representation}: Get multi-level representations by down sample detrended TS from step (1). For example, the level 1 representation is the original highest resolution detrended TS, and down sample level 1 by factor of 2 to generate the level 2 representation. This procedure is proceeded until the level $t$ representation is obtained, where $t$ is the total number of different levels in the multi-level framework. Note that higher level representations correspond to lower resolution TS.
%iterations that RobustDTW converges, usually $t$=3. Higher level representations correspond to lower resolution TS.
(3) \textbf{Projection and Upsampling}: Iteration starts from lowest level $t$. If current level is at $t$, call FastDTW to get warping index alignment and use current level representations as the base trend estimation; Otherwise, up-sample previous level's warping path by 2 and add extra searching width defined by parameter radius to generate the searching constraint for current level searching constraint, which is called projection. Also, we perform upsampling previous level trend estimation to current level.
(4) Time Warping Alignment by DTW: Refine the warping path by running DTW at current level with projected warping constrain.
(5) Temporal Graph Detrending: Generate graph using up-sampled trend estimate from (3) and refined DTW alignment from (4), and then update trend estimates and their distance at current level.
(6) Iterative Processing: Repeat (3)$\sim$(5) $t$ times, reduce the level per iteration until highest resolution.
(7) Return normalized distance.
In this procedure, steps (2) and (3) are unique in the multi-level framework, as they handle the interactions between adjacent levels.

\fi

%We have tested different implementations on multiple real-world datasets and found that the calculation time have been reduced by half from DTW to FastDTW and to by 1/3 from DTW to multi-level DTW. 


% \subsubsection{Handling Missing Values} \label{subsection:miss}
% deal with block missing values
% A straightforward method to handle missing values in DTW is simply removing all missing values with the same time range in DTW computation. However, it may not be appropriate since the missing segment may correspond to another segment in the other TS. In Fig.~\ref{fig:3-missing1}, the blue solid curves are \textbf{x}, \textbf{y} at higher resolution. There are two missing points on \textbf{y} which are marked by crosses. If these two points are not missing, then the optimal alignment learned from DTW will align them to their corresponding points on \textbf{x}, which are illustrated by the two blue dotted lines in Fig.~\ref{fig:3-missing1}. We want to exclude those points that are estimated to align with nans, such as $x_{1,right}^{high}$ in Fig.~\ref{fig:3-missing1}.

% Here we incorporate our multi-level framework and smooth assumption again to propose the following method to handle missing value. %As a simple example in Fig.~\ref{fig:3-missing1}, there are two TS \textbf{x} and \textbf{y} with time stamps, but there is a missing block in \textbf{y} (denoted by nans). 
% Our proposed scheme can be summarized as follows: (1) First, we perform downsampling by 2, average two adjacent points, recursively for both TS until the missing block disappears. We take average two adjacent points with following rule: If both points have values, then we take arithmetic mean as the result; if one of them are missing value and the other point has value, then their average is that value; if both of them are nans, then their average is still an nan. (2) In the lower resolution without missing values, we calculate the DTW and get the alignments, plotted in orange solid line in Fig.~\ref{fig:3-missing1}. (3) To estimate the alignment at higher resolution, we now look at the boundary of values and  nans. $x_1^{low}$ and $y_1^{low}$ are pair of aligned point in low resolution. $y_{1,left}^{high}$ has value and $y_{1,right}^{high}$ is a  nan, while both $x_{1,left}^{high}$ and $x_{1,right}^{high}$ have values. so we heuristically estimate alignment between them by find the argmin of $|x_{1,left}^{high}-y_{1,left}^{high}|$ and $|x_{1,right}^{high}-y_{1,left}^{high}|$. In this case, $|x_{1,left}^{high}-y_{1,left}^{high}|$ is smaller, so we align $x_{1,left}^{high}$ and $y_{1,left}^{high}$ in the high resolution. Following this rule, we can estimate the alignment in the boundary of nan blocks in the high resolution. In this way, we can remove the missing segment of current TS and its aligned counterparts on its peer TS. The same procedure is applied to multiple missing value blocks on both TS.

% % Then we can confine search constraint in cost matrix in Fig.~\ref{fig:3-missing2}. The shaded blue area are "removed" points caused by missing value. And the yellow area are updated constraint areas caused by missing values in high resolution. 
% %We can recursively perform upsampling to the highest resolution. 

% % missing value对应的点不再用time stamp硬性 align，而是考虑warping之后的对应点。讨论出从低分辨率到高分辨率时，nan边界的warping和constraint的迭代关系。

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.7\linewidth]{figs/3_misssing1b.pdf}
%     \caption{Illustration of handling block missing values in multi-level framework. Two TS \textbf{x} and \textbf{y} are plotted in high resolution (blue solid lines) and low resolution (orange dash lines), and their DTW alignments are also plotted with corresponding color. There are two missing points marked with crosses and their alignment are plotted with blue dash lines. The horizontal curly braces show that how to down sample and take average values from high resolution to low resolution.}
%     \label{fig:3-missing1}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figs/3_missing2.png}
%     \caption{Cost matrix for two TS \textbf{x} and \textbf{y} that have block missing values.}
%     \label{fig:3-missing2}
% \end{figure}

% 用户的prior input

% QS: 
% (1) Robust DTW https://yuque.antfin-inc.com/d3algo/alg-study/rdtw
% (2) general temporal/spatial operators?: https://yuque.antfin-inc.com/d3algo/alg-study/tdo#8480e148
% (3) graph detrending

%  ToDo: (1) Font in equations are not consistent in Methodology.
